Formal Analysis of UMTS Privacy

The ubiquitous presence of mobile communication devices and the continuous development of mo- bile data applications, which results in high level of mobile devices' activity and exchanged data, often transparent to the user, makes privacy preservation an important feature of mobile telephony systems. We present a formal analysis of the UMTS Authentication and Key Agreement protocol, using the applied pi-calculus and the ProVerif tool. We formally verify the model with respect to privacy properties. We show a linkability attack which makes it possible, for individuals with low-cost equipment, to trace UMTS subscribers. The attack exploits information leaked by poorly designed error messages.

==> identification.tex <==
\begin{figure}
\begin{tikzpicture}[node distance=4cm, auto,>=latex', thick]

	% We need to set at bounding box first. Otherwise the diagram
    % will change position for each frame.
    \path[use as bounding box] (4,3) rectangle (16,-1.0);
	%draw the two rectangles at the top of the vertical bars and the vertical bars
    \draw[elec] (6,2.5) node[format](ms){\small $K$, $SQN_{MS}$, $PK_{HN}$}-- (6,-0.5);
    \draw[elec] (10,2.5) node[format](sn){\small $K$, $SQN_{HN}$, $SK_{HN}$}-- (10,-0.5);
	\node [above=3mm] at (sn){SN/HN};
    \node [above=3mm] at (ms){MS};
	%draw the first arrow
	\node at (10.1,1)(startreq){};
    \node at (5.9,1)(endreq){};
    \path[elec,->](startreq) edge node[above] {\scriptsize IDENTITY\_REQUEST} (endreq);

	%draw mac fail arrow
    \node at (5.9,-0.0)(startresp){};
    \node at (10.1,-0.0)(endresp){};
    \path[elec,->](startresp) edge node[above] {\scriptsize IDENTITY\_RES$(\{IMSI\}_{PK_{HN}})$} (endresp);
  
\end{tikzpicture}
\caption{Identification procedure with use of public key to protect the user identity}
\label{id}
\end{figure}
